Combining Convolution and Recursive Neural Networks for Sentiment Analysis

This paper addresses the problem of sentence-level sentiment analysis. In recent years, Convolution and Recursive Neural Networks have been proven to be effective network architecture for sentence-level sentiment analysis. Nevertheless, each of them has their own potential drawbacks. For alleviating their weaknesses, we combined Convolution and Recursive Neural Networks into a new network architecture. In addition, we employed transfer learning from a large document-level labeled sentiment dataset to improve the word embedding in our models. The resulting models outperform all recent Convolution and Recursive Neural Networks. Beyond that, our models achieve comparable performance with state-of-the-art systems on Stanford Sentiment Treebank.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios
		Code prettying (Michael D. Adams)
		Two-column formats now balance the last page (ACM request)
		

==> chapters/background.tex <==
\section{Background}
\subsection{Word Embeddings}
A word embedding is a function mapping from words to their continuous vector representations.
The function encodes relevant syntactic and semantic features of words as relationships among their representation vectors.
Word embeddings are usually trained on large, unlabeled corpus~\cite{glove,word2vec} and then fine-tuned with respect to specific NLP tasks~\cite{treeLSTM,KimCNN}.
Pre-learned word representations have been applied widely and become the ``secret sauce'' for the success of recent NLP systems~\cite{Luong_betterword}.
\subsubsection{Matrix Representation of Sequences of Words}
Suppose that \(Z = \{e_0, e_1, \ldots e_m\}\) is a set input channels with each channel uses an independent word embedding, any sentence~\(s\) of length~\(n\) can be represented as a matrix.
For indexing, the first word in a sentence is word-\(0\)th.
In case the sentence is padded with dummy words, left padded dummy words are indexed by negative integers.

For any word embedding~\(e\), the vector presentation of the word-\(i\)th is denoted as~\(w^{(e)}_i \in \mathbb{R}^{d_e}\).
The vector presentation of word-\(i\)th through the set of input channels \(Z\) is expressed as follow:
\begin{align}
 x_i &= w^{(e_0)}_i \ominus w^{(e_1)}_i \ominus  \ldots \ominus w^{(e_m)}_i&\label{concat-emb}
\end{align}
In Eq.\eqref{concat-emb}, \(\ominus\) is concatenation operator which results in the vector \(x_i \in \mathbb{R}^{d}\) with \(d = \sum_{e \in Z} d_e\).
Any sequence of words in the sentence which starts at word-\(i\)th and ends at word-\(j\)th is presented as the following matrix:
\begin{align}
X_{i:j} &= x_i \oplus x_{i+1} \oplus \ldots \oplus x_j &\label{concat}
\end{align}
In Eq.\eqref{concat}, \(\oplus\) is concatenation operator which results in the matrix \(X_{i:j} \in \mathbb{R}^{d \times (j-i+1)}\).
\subsection{Convolution and Pooling}\label{sec:cnn}
Convolution Neural Networks (CNNs) have been proven to be effective models for the task of sentence-level sentiment analysis~\cite{KimCNN, DCNN,2-layer-cnn}.
Convolution Neural Networks are commonly constructed by stacking up multiple convolution, pooling and fully connected layers.
\subsubsection{Convolution Layer}\label{conv-layer}
Given that \(F\) is the set of all filters of the convolution layer, for any filter \(v \in F\) which has window size \(l\) and set of parameters \(\theta^{(v)} = \{ W^{(v)}, b^{(v)} | W^{(v)} \in \mathbb{R}^{d \times l}, b^{(v)} \in \mathbb{R}\}\), filter \({v}\) is applied on any sequence of word-\(i\)th to word-\((i+l-1)\)th through the following equation:
\begin{align}
c^{(v)}_j &= f(W^{(v)} \otimes X_{i:i+l-1} + b^{(v)}) &\label{filter}
\end{align}
In Eq.\eqref{filter}, operator \(\otimes\) is the Hadamard product~\cite{element-prod}.
\(b \in \mathbb{R}\) as bias term and \(f\) is an activation function.
For indexing, \(j = i + x\) with \(x \in \mathbb{N}\) and \(0 \leq x < l\).
If half-padding policy is employed then \(j = i + \floor{\frac{l}{2}}\).

By slicing the filter \(v\) through the sentence (i.e. applying the filter \(v\) on different sequences of length \(l\) along the sentence) we can get vector \(c^{(v)} = [c^{(v)}_0, c^{(v)}_1~\cdots]\) which is a feature map of the sentence~\(s\).
The length of the feature map \(c^{(v)}\) depends on the length of the input sentence.
Additionally, the length of \(c^{(v)}\) also depends on the way which filter \(v\) was slided through the sentence and its window size \(l\)~\cite{conv-arith}.
In summary, each filter produces a variable-length feature map of the sentence.
As a result, when applying a convolution layer on a sentence, we get a set of variable-length feature maps.
\subsubsection{Max Pooling Layer}
For dealing with the problem of variable-length feature maps, several types of max pooling layer were employed.
In general, given a input vector \(i\), a \(k\)-max pooling layer reduces the size of vector \(i\) by extracting the largest \(k\) entries from \(i\).
In case \(k = 1\) the pooling layer is called max-over-time pooling~\cite{nlp-scratch,KimCNN}.
Apart from being treated as a hyper-parameter, \(k\) can also be parameterized with respect to the length of the input sentence, in which case, the pooling layer is called dynamic k-max pooling~\cite{DCNN}.
\subsection{Recurrent Neural Network}
By definition, Recurrent Neural Networks are any Neural Networks which have at least a recurrent connection~\cite{rnn-def}.
Recurrent Neural Networks have been proven to be effective network architecture when applied on the type of problems whose output is determined by a variable-length input sequence~\cite{speech-lstm,SutskeverVL14,mikolov-nlm}.
\subsubsection{Vanilla Recurrent unit}\label{sec:vanilla-rnn}
Denoting input sequence as \(I = \{i_0,\ldots,i_n\}, \forall t, i_t \in \mathbb{R}^n\), Vanilla Recurrent unit is expressed as the following recursive formula~\cite{treeLSTM}:
\begin{align}
h_t &= tanh(Wi_t + Uh_{t-1} + b)&
\end{align}
For sentence-level sentiment analysis, \(h_n\) is treated as output of the network.
In theory, Vanilla Recurrent Neural Network is Turing-Complete~\cite{rnn-turing-complete} but hard to train (especially on long input sequence) due to the problems of exploding and vanishing gradient~\cite{Bengio1994}.
Long Short Term Memory unit (LSTM)~\cite{originLSTM} unit was invented to mitigate the problem of vanishing gradient.
\subsubsection{Long Short Term Memory unit}\label{sec:lstm}
Long Short Term Memory unit is expressed as the following recursive formula~\cite{treeLSTM}:
\begin{align}
w_t &= \sigma\left(W^{(w)}i_t + U^{(w)}h_{t-1} + b^{(w)}\right) \label{eq:lstm-input-gate}&\\
f_t &= \sigma\left(W^{(f)}i_t + U^{(f)}h_{t-1} + b^{(f)}\right) \label{eq:lstm-forget-gate}&\\
o_t &= \sigma\left(W^{(o)}i_t + U^{(o)}h_{t-1} + b^{(o)}\right) \label{eq:lstm-output-gate}&\\
u_t &= tanh\left(W^{(u)}i_t + U^{(u)}h_{t-1} + b^{(u)}\right) \label{eq:lstm-update-gate}&\\
c_t &= r_t \odot u_t + f_t \odot c_{t-1} \label{eq:longterm-mem}&\\
h_t &= o_t \odot tanh(c_t) \label{eq:temperal-mem}&
\end{align}
The operation \(\odot\) denotes the element-wise vector product.
Traditionally, \(w_t\), \(f_t\) and \(o_t\) are called input/write gate, forget/deallocate gate and output/read gate respectively and \(c_t\) is called memory cell.
Intuitively, we can interpret how the network works as follow:
in the above formula, \(h_{t-1}\) can be viewed as a short-term memory of the network;
\(u_t\) is the information extracted from in current input \(i_t\) and the short-term memory \(h_{t-1}\);
write gate \(w_t\) decides which information from \(u_t\) will be written into the memory cell \(c_t\);
forget gate \(f_t\) decides which information will be preserved on memory cell \(c_t\);
and \(o_t\) decides which information will be read from the memory cell \(c_t\), which will produce the short-term memory (or output) \(h_t\).
\subsection{Recursive Neural Network}\label{sec:recursive-nn}
In most cases, to understand a sentence, we must understand the phrases composing it, and to understand a phrase, we must understand the phrases and words composing the phrase.
Recursive Neural Networks were mainly inspired by this idea~\cite{treeLSTM}.
Given a sentence and its parse tree, a Recursive Neural Network composes the vector presentation of the sentence by applying its composition function at each node of the parse tree in a bottom-up manner.
Note that, Recurrent is a special case of Recursive Neural Network where the parse tree is a linear chain.
For demonstration, parse tree of the phrase ``is a fluffy cat'' and its composing process using a Recursive Neural Network are illustrated in Fig.\ref{fig:example-parse} and Fig.\ref{fig:example-compose} respectively~\cite{tag-embedding-rnn}.
\begin{figure}[]
	\centering
	%\includegraphics[scale=0.4]{figure/example-parse}
	\input{figure/cattree.tikz}
	\caption[Constituency parse tree for the phrase ``is a fluffy cat'']{Constituency parse tree for the phrase ``is a fluffy cat''.}
	\label{fig:example-parse}
\end{figure}
\begin{figure}[]
	\centering
	% \includegraphics[scale=0.3]{figure/example-compose}
	\input{figure/catcompile.tikz}
	\caption[Applying Recursive Neural Network on the phrase ``is a fluffy cat'']{Applying Recursive Neural Network on the Constituency parse tree of the phrase ``is a fluffy cat''.
		The composition function of this network is denoted as \textbf{g}.}
	\label{fig:example-compose}
\end{figure}

One of the most successful Recursive Neural Networks are Tree-LSTMs~\cite{treeLSTM}.
The core idea behind the design of Tree-LSTMs are to generalize the LSTM for tree-structured inputs.
Tree-LSTMs were able to achieve state-of-the-art performance on two tasks: predicting the semantic relatedness of two sentences (SemEval 2014, Task 1~\cite{SemeEvalTask1}) and sentiment classification (Stanford Sentiment Treebank~\cite{socher2013recursive}).
\subsubsection{Constituency Tree-LSTM}\label{treelstm}
Let \(d\) be the size of the input vectors, \(r
\) be the size of the memory cell and \(z\) be the number of sentiment classes.
\paragraph{Leaf module}
Given any input vector \(x \in \mathbb{R}^d\), the calculation steps inside the leaf module can be expressed as follow:
\begin{align}
o &= \sigma{\left( W^{(o)} x + a^{\left(o\right)}\right)} & \\
c &= W^{(c)} x + a^{(c)} & \\
h &= o \odot \tanh{\left(c\right)} &
\end{align}
In this module, \(W^{(o)}, W^{(c)} \in \mathbb{R}^{r \times d}\) and \(a^{\left(o\right)}, a^{(c)} \in \mathbb{R}^r\).
\paragraph{Composer module}
Given the input vectors \({h_l}\), \({c_l}\) from the left child node and \({h_r}\), \({c_r}\) from the right child node, the calculation steps inside the composer module can be expressed as follow:
\begin{align}
i &= \sigma{ \left(U_l^{(i)} h_{l} + U_r^{(i)} h_{r} + b^{(i)} \right) } &\\
f_{l} &= \sigma{\left(U_{l}^{(l)} h_{l} + U_{r}^{(l)} h_{r} + b^{(f)}\right)} & \\
f_{r} &= \sigma{\left(U_{l}^{(r)} h_{l} + U_{r}^{(r)} h_{r} + b^{(f)}\right)} & \\
o &= \sigma{\left( U_l^{(o)} h_{l} + U_r^{(o)} h_{r} + b^{(o)}\right)} &\\
u &= \tanh{\left( U_l^{(u)} h_{l} + U_r^{(u)} h_{r} + b^{(u)}\right)} &\\
c &= i \odot u + f_{l} \odot c_{l} + f_{r} \odot c_{r} & \\
h &= o \odot \tanh{\left(c\right)} &
\end{align}
In this module, for any \(j \in \{i, l, r, o, u\}\) and \(x \in \{l, r\}\), \(U_x^{(j)} \in \mathbb{R}^{r \times r}\) and \( b^{(j)} \in \mathbb{R}^r\).
\paragraph{Output module}
Denoting sequence of words spanned by a sub-tree rooted at node \({j}\) as \({\{x\}_j}\).
Given \({h_j}\) is the \({h}\) output of node \({j}\), the prediction at node \({j}\) can be computed by the output module as follow:
\begin{align}
\hat{p_{\theta}}(y \mid \{x\}_j ) &= softmax( W^{(s)} h_j + b^{(s)}) & \\
\hat{y_j} &= \underset{y}{\mathrm{argmax}} \; \hat{p_{\theta}}(y \mid \{x\}_j ) &
\end{align}
In this module, \(W^{(s)} \in \mathbb{R}^{z \times r}\) and \( b^{(s)} \in \mathbb{R}^z\).
\paragraph{Composing sentence}
Given any sentence, its parse tree and a word embedding, each word in the sentence is mapped to a representation vector.
For any non-leaf node, composer module is applied recursively and for any leaf node, the leaf module is applied on the vector representation of the corresponding word.
Finally, we can apply the output module on any node in the parse tree.
Recursive Neural Networks have several advantages over Recurrent Neural Networks:
\begin{itemize}
	\item In case the input sequence belongs to a recursively defined language, given only a small subset of the data with limited length sentences, tree structures model have better ability to generalize comparing to sequential ones.
	However, when the limited length of sentences in the training data is increased, the advantage of tree over sequential models decreases fast~\cite{bowman-treevslstm}.
	\item Tree can breaks down complicated sentences into simpler phrases, which makes it easier for generalization~\cite{knowledge-matter}~\cite{need-tree}.
	\item Some features which are far apart when a sentence is presented as sequence become closer when it is presented as tree~\cite{need-tree}.
\end{itemize}


==> chapters/challenges.tex <==
\section{Challenges}
\subsection{Convolution and Pooling}\label{sec:cnn-weak}
Although max pooling layer largely simplified the network (which is good for preventing over-fit), this solution have a clear disadvantage.
By down-sampling a feature map, although the resulted vector still contains information about the existence of a feature, it is likely that the information about the position of the feature is ignored, especially for the case of max-over-time pooling.
\subsection{Recursive Neural Network}\label{sec:recursive-nn-weak}
Tree-LSTMs also have some drawbacks, including:
\begin{itemize}
	\item Sentences can be wrongly parsed, especially when comments are expressed in informal language.
	The performance of the system depends on the parser being used.
	\item At their leaf-module, Tree-LSTMs have only a simple logistic regression layer on top of the vector presentation of a single word at that position.
	The simple leaf-module of Tree-LSTMs might be its weakness when dealing with the problem of words ambiguity.
	This weakness becomes even more severe when the sentence is wrongly parsed. 
\end{itemize}
\subsection{Word Embeddings}\label{sec:word-weak}
There are many words (e.g. ``B-rated'', ``Batman'', ``Nolan'', ``cartoonlike'') which rarely appears in regular documents but more often in movie reviews.
These words might not appear or not have good vector representations in the pre-trained Glove Common Crawl.

Additionally, the ways people use words in movie reviews might be different from their usage in general documents.
For example, the vector presentations of ``sympathy'' and ``disappointed'', or ``boom'' and ``insult'' are very close to each other in Glove Common Crawl but if we have to predict the sentiment of a movie comment which has one of these words, they should be distinctive.

Noticeably, many experiments~\cite{treeLSTM, KimCNN} have shown that modifying word embeddings during the training process help improving the performance of Deep Learning systems.
Although this method improves models' performance, it can harm generalization by updating only words which appear in the training set and non-related words which only appear in the test set.

==> chapters/method.tex <==
\section{Combining Convolution and Recursive Neural Networks}%\label{sec:cnn-treelstm}
For composing fixed size presentation vectors of a sentence given a set of variable-length feature maps, one intuitive solution would be to apply Recurrent Neural Networks which have been done by Wang et al.~\cite{cnn-rnn}.
Another solution would be to utilize Recursive Neural Networks.

Different from the leaf module of Constituency Tree-LSTM, CNNs'~\cite{KimCNN,DCNN,2-layer-cnn} first convolution layer have hundreds of filters, each produces a feature map of the sentence by sliding through it with window sizes 3 to 5 words.
Filters with large context window might help CNNs to mitigate the problem of words ambiguity and to capture phrase-level features.
We think this is the reason why CNNs can outperform TreeLSTMs~\cite{KimCNN}, even when it has little regard for the positions of features. 

We combined Convolution Neural Networks with Constituency Tree-LSTM.
We hypothesized that the convolution layer helps Constituency Tree-LSTM to mitigate the problem of lacking local context and words ambiguity at leaf nodes.
Additionally, using Constituency Tree-LSTM to combine the feature maps produced by the convolution layer might be a better choice compared to using max pooling layers.
\subsection{Model}
Our model has three modules: word embeddings, convolution layer, and Constituency Tree-LSTM.
\begin{figure} [H]
	\centering
	\input{figure/cnntreelstm.tikz}
	\caption[qwerty]{CNN-Tree-LSTM}
\end{figure}
\subsubsection{Convolution Layer}
Convolution layer is described in Sec.~\ref{conv-layer}.
For working with Constituency Tree-LSTM, after going through the convolution layer, the parse tree structure of sentence \(s\) must be applied on the output of the convolution layer. 
For this purpose, we constrained all the feature maps produced by the convolution layer to have the length equal to that of the sentence \(s\) (which is \(n\) in this case).
Additionally, all filters in \(F\) are restricted to have odd window sizes and being applied on the sentence according to half padding, unit strides policy~\cite{conv-arith}.
These conditions entail \({\forall u \in F,  c^{(u)} \in \mathbb{R}^n}\)~\cite{conv-arith}.

Suppose the size of the set of filters \(F\) is \(m\), all the feature maps produced by the set of filters is then concatenated into one matrix \(P \in \mathbb{R}^{m \times n}\), of which each row is a feature map.
After that, the column vectors of \(P\) are treated as input vectors for the Constituency Tree-LSTM.
\subsubsection{Constituency Tree-LSTM}
The definition of Constituency Tree-LSTM which is described in Sec.~\ref{treelstm} is reused.
The only difference is that for any word-\(i\)th in the sentence, the vector representation of it is the \(i\)th-column of the matrix \(P\) produced by the convolution layer.
This means the size of any input vector for the Constituency Tree-LSTM is equal to the number of filters \(m\).
\subsection{Model Enhancement}
We observed that the available amount of document-level labeled sentiment data (e.g., Amazon Reviews dataset~\cite{amazon-reviews} has 83.68 million reviews) is gigantic compared to the amount of sentence or phrase-level sentiment data (e.g., Stanford Sentiment Treebank~\cite{socher2013recursive} which has 8,544 sentences in its training set, even it is the biggest sentence-level sentiment analysis dataset).
Although there are some attempts to do transfer learning~\cite{group-instance, re-embedding} (i.e., training on large document-level sentiment dataset then fine-tuning and/or test on sentence-level sentiment dataset), their performances are not high when being evaluated on Stanford Sentiment Treebank~\cite{group-instance}.

We utilized Glove~\cite{glove} method to do transfer learning.
We hypothesized that by training Glove on review documents, especially movie or book reviews, we can capture more rare words and also the different way that people use words (or different word relationships) to express their opinions on movies or books.
This might help our models achieving better generalization when training on small sentence-level sentiment dataset (e.g. Stanford Sentiment Treebank~\cite{socher2013recursive}).
